Learning Team Decisions

In this paper, we treat linear quadratic team decision problems, where a team of agents minimizes a convex quadratic cost function over $T$ time steps subject to possibly distinct linear measurements of the state of nature. We assume that the state of nature is a Gaussian random variable and that the agents do not know the cost function nor the linear functions mapping the state of nature to their measurements. We present a gradient-descent based algorithm with an expected regret of $O(\log(T))$ for full information gradient feedback and $O(\sqrt(T))$ for bandit feedback. In the case of bandit feedback, the expected regret has an additional multiplicative term $O(d)$ where $d$ reflects the number of learned parameters.

==> sections/problem_old.tex <==
Armed with Proposition~\ref{prop:linear} we restrict our attention to searching among linear policies, and define the equivalent problem:
\begin{problem}
\label{prob:stoch_linear}
The stochastic linear-quadratic optimal distributed decision-making problem with linear policies $K_1, \ldots, K_N$ is defined by the following optimization problem and assumptions \ref{ass:bounded_moments} and \ref{ass:strongly_convex}.
\begin{equation}
	\begin{aligned}
		\underset{K\in \K}{\text{minimize}} \quad & J(K) = \E [\|z\|_2^2]\\
		\text{subject to:}\quad & z = Hx + Du\\
		& y_i = C_ix + v_i \\
		& u_i = K_iy_i, \quad i = 1, \ldots, N.
	\end{aligned}
	\label{eq:stoch_prob_linear}
\end{equation}
In \eqref{eq:stoch_prob_linear}, $x$ and $v$ are independent, zero-mean random variables taking values in $\R^n$ and $\R^p$ respectively.
The actions $u_i$ are stochastic variables taking values in $\R^{m_i}$, $m = m_1 + \cdots + m_N$.
The performance quantity $z$ is a stochastic variable taking values in $\R^l$ and $H \in \R^{l \times n}$, $D \in \R^{l \times m}$, $C_i \in \R^{p_i \times n}$.
$\K$ is the set of real-valued block-diagonal matrices of appropriate dimensions,
\begin{multline}
    \K := \{K \in \R^{n\times m}: K = \Diag(K_1, \ldots, K_N), \\ K_i \in \R^{m_i \times p_i} \}.
    \label{eq:K}
\end{multline}
\begin{assumption}
\label{ass:bounded_moments}
$x$ and $v$ have finite covariance matrices $\E [xx^\top] = V_{xx}$ and $\E [vv^\top] = V_{vv}$ and bounded fourth order moments so that $\E [(x^\top x)^2] \leq \kappa_x$ and $\E [(v^\top v)^2] \leq \kappa_v$.
\end{assumption}
\begin{assumption}
\label{ass:strongly_convex}
\[
    \sigma_\text{min}(D^\top D) (\sigma_\text{min}(CV_{xx}C^\top) + \sigma_\text{min}(V_{vv})) > 0.
\]
\end{assumption}
\end{problem}

Assumption~\ref{ass:bounded_moments} is motivated by the fact that the variance of an estimator of the derivative $\frac{\partial}{\partial K}J(K)$ will contain fourth-order moments. Assumption \ref{ass:strongly_convex} is used to restrict our search of $K$ to a bounded set in Proposition~\ref{prop:stoch_bound_K}. It is also related to \eqref{eq:stoch_prob_linear} being strongly convex, which is summarized in Proposition~\ref{prop:strongly_convex}. 

We wish to learn the optimal decisions to Problem~\ref{prob:stoch_linear} in a distributed fashion using repeated interactions as outlined in Algorithm~\ref{alg:learn}.

\begin{algorithm}[tb]
   \caption{Learning with repeated interactions.}
   \label{alg:learn}
\begin{algorithmic}
    \FOR{$t=1$ {\bfseries to} $T$}
       \STATE Sample $(x_t, v_t) \sim (x, v)$.
        \STATE Agents $1, 2, ..., N$ observes $y^t_1, \ldots, y^t_N$, respectively.
        \STATE The agents play $K^t_1, \ldots, K^t_N$, respectively, and incur a cost $ J_t(K_t) := \|z_t\|_2^2$.
        \STATE Each agent $i$ observes either
            \begin{itemize}
        \item the partial derivative, $\frac{\partial}{\partial K_i} (z_t)^\top z_t$, in the gradient-feedback setting,
        \item or the incurred loss, $\|z_t\|_2^2$, in the bandit-feedback setting
    \end{itemize}
    \STATE The agents update their policies $K_i^{t+1}$.
    \ENDFOR
\end{algorithmic}
\end{algorithm}

We introduce the following assumption on $\|K\|_2$.
\begin{assumption}
    \label{ass:bk}
    A bound $b_K$ on $\|K\|_2$ is supplied by an oracle.
\end{assumption}
Let $K^\star$ be the best policy in hindsight,
\begin{equation}
    K^\star = \argmin_{K\in\K, \|K\|_2 \leq b_K}\sum_{t=1}^T J_t(K).
    \label{eq:Kstar}
\end{equation}
We measure performance as expected regret, 
\begin{equation}
    \E[{R}(T)] = \E\left[\sum_{t=1}^T J_t(K_t) - \sum_{t=1}^T J_t(K^\star) \right].
    \label{eq:regret}
\end{equation}

==> sections/robust.tex <==
In this section we propose a reduction of the robust team-decision problem, defined below, to an equivalent stochastic problem and apply the previous results.
\begin{equation}
	\begin{aligned}
		\underset{\mu}{\text{minimize}} \sup_{0 \neq x \in \R^n} \quad & \||z\|_2^2 / \|x\|_2^2\\
		\text{subject to:}\quad & z = Hx + Du\\
		& y_i = C_ix \\
		& u_i = \mu_i(y_i), \quad i = 1, \ldots, N,
	\end{aligned}
	\label{eq:robust_prob}
\end{equation}
where $u_i \in \R^{m_i}$, $m = m_1 + \cdots + m_N$, $C_i \in \R^{p_i\times n}$, $H \in \R^{l\times n}$ and $D \in \R^{l\times m}$ such that $D^\top D \in \S^m_{++}$. The above problem represent a game where the team $u_1, \ldots, u_N$ plays against nature $x$. 

\begin{theorem}[Theorem 1 in \cite{Gattami2012Robust}]
Let $z = Hx + Du$ with $D^\top D \succ 0$. Suppose that 
\[
    \inf_\mu \sup_{0 \neq x\in \R^N} \|z\|_2^2 / \|x\|_2^2 = \gamma^\star < \infty.
\]
Then there exist linear decisions $\mu_i(C_ix) = K_i C_i x$, $i = 1, \ldots, N$, that achieves the value of the game, $\gamma^\star$.
\end{theorem}

We can again exploit that $K=0$ is a feasible strategy and bound the norm of an optimal $K^\star$.

\begin{proposition}
    \label{prop:robust_bound_K}
    Let $z = Hx + Du$ with $D^\top D \in \S^m_{++}$. Then $\gamma^\star \leq \|H\|_2$ and there exists an optimal $K^\star$ such that
    \begin{equation}
        \|K^\star\|_2 \leq 2 \frac{\|H\|_2}{\sigma_{\text{min} > 0}(D)\sigma_{\text{min} > 0}(C)}.
        \label{eq:robust_bound_K}
    \end{equation}
\end{proposition}

The following section cast the robust team-decision problem as a stochastic team-decision problem. 
\subsection{Reduction to a Stochastic Team-Decision Problem}
Let $\gamma > \gamma^\star$, then the game has a value less than $\gamma$ if and only if for all $x \in \R^n$, $\|z\|^2_2 \leq \gamma \|x\|_2^2$. Let
\[
    Q := \bmat{H & D}^\top \bmat{H & D},
\]
then $\|z\|^2_2 \leq \gamma \|x\|_2^2$ for all $x$ is equivalent to the inequality
\[
    \bmat{I \\ KC}^\top Q \bmat{I \\ KC} \preceq \gamma I.
\]

We can thus construct a semi-definite program whose solution $K^\star$ also solves \eqref{eq:robust_prob}.
\begin{equation}
\begin{aligned}
    \underset{K \in \K, s}{\text{minimize}} \quad & s \\
    \text{subject to:} \quad & \bmat{I \\ KC}^\top Q \bmat{I \\ KC} \preceq s I,
\end{aligned}
\label{eq:robust_sdp}
\end{equation}
where 
\begin{multline*}
\K = \{ K \in \R^{m\times p} : K = \Diag(K_1, \ldots, K_N), \\
    \|K_i\|_2 \leq b_{K_i}, K_i \in \R^{m_i\times p_i}\}
\end{multline*}
is the set of block-diagonal matrices whose $i$:th block has $m_i$ rows, $p_i$ columns and induced norm bounded by $b_{K_i}= 2 \frac{\|H\|_2}{\sigma_{\text{min} > 0}(D)\sigma_{\text{min} > 0}(C_i)}$. The semi-definite program \eqref{eq:robust_sdp} satisfies Slater's condition so strong duality holds, with the dual being, \cite{Boyd2004Convex},

\begin{equation}
    \max_{X \in \X}\min_{K \in \K} \Tr \left( \bmat{I \\ KC}^\top Q \bmat{I \\ KC}X \right).
    \label{eq:robust_sdp_dual}
\end{equation}

In \eqref{eq:robust_sdp}, the set $\X = \{ S \in \S_+^{n\times n}: \Tr S = 1\}$ is the set of positive semi-definite matrices whose diagonal elements sum up to one. Since \eqref{eq:robust_sdp_dual} is a convex-concave function over compact sets, we can apply Von Neumann's minimax theorem and conclude the existence of a Nash equilibrium $(K^\star, X^\star)$. The value of \eqref{eq:robust_sdp_dual} at the Nash equilibrium is
\begin{multline*}
    \Tr \left(\bmat{I \\ K^\star C}^\top Q \bmat{I \\ K^\star C}X^\star\right) \\ = \E \left[x^\top \bmat{I \\ K^\star C}^\top Q \bmat{I \\ K^\star C}x\right],
\end{multline*}
where $x$ is any zero-mean random variable with covariance $\E [xx^\top] = X^\star$, for example we could take $x \sim \N(0, X^\star)$. This motivates the learning situation where nature plays according to the Nash equilibrium $X^\star$ and the players $u_1, \ldots, u_N$ have to learn the optimal strategies $K_1^\star, \ldots, K_N^\star$. If we impose that $\E[ (x^\top x)^2] = \kappa_x \leq \infty$, then we can directly use algorithms~\ref{alg:fg_feedback} or \ref{alg:bandit_feedback} depending on whether the players learn the gradient or only the realized cost. The caveat is that the problem is not necessarily strongly convex, we thus have to base our analysis on Theorem~\ref{thm:GD_convex}.

\begin{theorem}[Partial-Gradient Feedback: Robust Problem]
\label{thm:robust_fg_feedback}
Assume that Assumption~\ref{ass:bk} holds. Running Algorithm~\ref{alg:fg_feedback} with step-size $\eta_t = \frac{2\sqrt{\max\{m, p\}}}{b_G\sqrt t}$ on the stochastic relaxation of the robust team-decision problem, has bounded expected regret against the optimal policy $K^\star$ defined in \eqref{eq:Kstar}. The bound is given by
\begin{equation}
    \sum_{t=1}^T \E[J_t(K_t) - J_t(K^\star)] \leq 4 \sqrt{\max\{m, p\}}(b_K^2 + b_G^2)\sqrt{T}
    \label{eq:robust_fg_regret}
\end{equation}

The constant $b_G$ in \eqref{eq:robust_fg_regret} is given by
\begin{equation*}
    b^2_G = 4\|D\|_2^2(\|H\|_2 + b_K\|D\|_2\|C\|_2)^2\|C\|_2^2\\
    \kappa_x
\end{equation*}
\end{theorem}

\begin{proof}
The result follows from substituting $v = 0$ and $b_K$ into the gradient estimate from Lemma~\ref{lemma:stoch_bound_dJ} and applying Theorem~\ref{thm:GD_convex} with step-sizes $\{\eta_t\}$. Finally we apply the upper bound $\sum \frac{1}{\sqrt t}\leq 2 \sqrt{T}$.

The term $\min\{m, p\}$ comes from bounding the diameter $d_K$ in Frobenius norm using the relationship $\|A\|_F \leq \sqrt{r} \|A\|_2$, where $r$ is the rank of $A$.
\end{proof}
\begin{theorem}[Bandit Feedback: Robust Problem]
\label{thm:robust_bandit_feedback}
Assume that Assumption~\ref{ass:bk} holds and let the step sizes $\{\eta_t\}$ and exploration parameters $\eta_t$ be
\begin{equation}
\begin{aligned}
    \eta_t  & = \frac{\left(4 \min (m, p)b_K^2 \right)^{2/3}}{\left(\sum_{i=1}^N m_i^2 p_i^2 \right)^{1/3}} \frac{1}{t^{1/3}}\\
    \epsilon_t & =\left(4 \min (m, p)b_K^2 \right)^{1/6}\left(\sum_{i=1}^N m_i^2 p_i^2 \right)^{1/6} \frac{1}{t^{1/6}}.
\end{aligned}
\label{eq:robust_params}
\end{equation}

Running Algorithm~\ref{alg:bandit_feedback} with step-sizes $\{\eta_t\}$ and exploration parameters $\{\epsilon_t\}$ as defined above on the stochastic relaxation of the robust team-decision problem, has bounded expected regret against the optimal policy $K^\star$ defined in \eqref{eq:Kstar}. The bound is given by
\begin{multline}
    \sum_{t=1}^T \E[J_t(K_t + \R_t \mathcal E_t) - J_t(K^\star)] \leq \\
    \frac{3}{2}\left(4 \min \{m, p\}b_K^2 \right)^{1/3}\left(\sum_{i=1}^N m_i^2 p_i^2 \right)^{1/3}  M T^{2/3}
    \label{eq:robust_bandit_regret}
\end{multline}
where 
\[
    M = 1 + (\|H\|_2 + \|D\|_2\|C\|_2b_K)^4\kappa_X + \|D\|_2^2\|C\|_2^2.
\]
\end{theorem}
\begin{proof}
Modifying Lemma~\ref{lemma:stoch_bound_Gtilde} for the case where $v = 0$, we see that the variance bound for the gradient oracle becomes
\[
    (\tilde b^t_G)^2 = \left( \|H\|_2 + \|D\|_2\|C\|_2 b_K\right)^4\kappa_X \sum_{i=1}^N m_i^2 p_i^2 / (\epsilon_t)^2.
\]

To apply Theorem~\ref{thm:GD_convex} we need a bound on the diameter of $\K$, $d_K$. By equivalence of norms we have $\|K\|_F \leq \sqrt{\min \{m, p\}}\|K\|_2$, so we take $d_K = 2\sqrt{\min \{m, p\}}\|K\|_2$. Similarly to the proof of Theorem~\ref{thm:bandit_feedback} we have
\[
    \E [J_t(\tilde K_t)] \leq \E[J_t(K^t)] + (\epsilon_t)^2\|D\|_2^2\|C\|_2^2.
\]

We bound the expected regret by
\begin{multline*}
\sum_{t=1}^T \E[J_t(K_t + \R_t \mathcal E_t) - J_t(K^\star)] \\ \leq \sum_{t=1}^T \E[J_t(K_t) - J_t(K^\star)] + \|D\|_2^2\|C\|_2^2\sum_{t=1}^T(\epsilon_t)^2
\end{multline*}
Applying Theorem~\ref{thm:GD_convex} with $d_K$, $\eta_t$, $\tilde b_G^t$ from \eqref{eq:robust_params} together with the bound $\sum_{t=1}^T \frac{1}{t^{1/3}} \leq \frac{3}{2} T^{2/3}$ completes the proof.
\end{proof}

